Real-Time Seizure Detection using EEG: A Comprehensive Comparison of Recent Approaches under a Realistic Setting

Electroencephalogram (EEG) is an important diagnostic test that physicians use to record brain activity and detect seizures by monitoring the signals. There have been several attempts to detect seizures and abnormalities in EEG signals with modern deep learning models to reduce the clinical burden. However, they cannot be fairly compared against each other as they were tested in distinct experimental settings. Also, some of them are not trained in real-time seizure detection tasks, making it hard for on-device applications. Therefore in this work, for the first time, we extensively compare multiple state-of-the-art models and signal feature extractors in a real-time seizure detection framework suitable for real-world application, using various evaluation metrics including a new one we propose to evaluate more practical aspects of seizure detection models. Our code is available at https://github.com/AITRICS/EEG_real_time_seizure_detection.

==> Sections/Table_ResNetFeatExtrac.tex <==
\begin{table*}[ht!]
	\footnotesize
	\centering
	\caption{Real-time seizure detection performance on \textbf{Bipolar} TUH EEG dataset trained with each different \textbf{signal process feature extractor} on \textbf{ResNet-short + LSTM}. The results were averaged over $5$ runs.}
	\label{resnet_feature}
	\begin{tabular}{c|cccc}
		\toprule
		Methods & AUROC & AUPRC & TPR & TNR\\
		\midrule
		\textbf{Raw} & \textbf{0.92 $\pm$ 0.00}  &  \textbf{0.91 $\pm$ 0.00}  &  \textbf{0.83 $\pm$ 0.02}  &  \textbf{0.85 $\pm$ 0.01} \\
		SincNet & 0.83 $\pm$ 0.01 & 0.81 $\pm$ 0.02 & 0.71 $\pm$ 0.02 & 0.79 $\pm$ 0.02  \\
		Frequency Bands & 0.91 $\pm$ 0.01 & 0.88 $\pm$ 0.02 & 0.81 $\pm$ 0.01 & 0.83 $\pm$ 0.02  \\
		STFT  & 0.9 $\pm$ 0.03 & 0.88 $\pm$ 0.02 & 0.84 $\pm$ 0.0 & 0.81 $\pm$ 0.05  \\
		Downsampled Raw  & 0.91 $\pm$ 0.01 & 0.89 $\pm$ 0.01 & 0.83 $\pm$ 0.04 & 0.82 $\pm$ 0.02   \\
		LFCC  & 0.86 $\pm$ 0.02 & 0.84 $\pm$ 0.01 & 0.8 $\pm$ 0.03 & 0.78 $\pm$ 0.04  \\
		\bottomrule
	\end{tabular}
\end{table*}

==> Sections/Table_Result_Calibration.tex <==
\begin{table}[h!]
	\small
	\centering
	\caption{\textbf{Calibration} of each real-time seizure detection model using temperature scaling.}
	\label{calibration}
	\begin{tabular}{c|c}
		\toprule
		Methods & ECE \\
		\midrule
% 		CNN2D+BLSTM & 88.9 $\pm$ 1.6 & 88.9 $\pm$ 1.6 & 88.9 $\pm$ 1.6 & 88.9 $\pm$ 1.6 & 88.9 $\pm$ 1.6 \\
		CNN2D + LSTM &  $\pm$  \\
		CNN2D (ResNet) + LSTM &  $\pm$  \\
		CNN2D (ResNet with Dilation) + LSTM &  $\pm$  \\
		CNN2D (MobileNet) + LSTM &  $\pm$  \\
		CNN2D (AlexNet) + LSTM &  $\pm$  \\
		CNN2D (DenseNet) + LSTM &  $\pm$  \\
		CNN2D (SeizureNet) + LSTM &  $\pm$  \\
		\midrule
% 		CNN1D+BLSTM & 88.9 $\pm$ 1.6 & 88.9 $\pm$ 1.6 & 88.9 $\pm$ 1.6 & 88.9 $\pm$ 1.6 & 88.9 $\pm$ 1.6 \\
		CNN1D + LSTM &  $\pm$  \\
		CNN1D (ChronoNet) + LSTM &  $\pm$  \\
		\midrule
		Feature Transformer &  $\pm$  \\
		\midrule
		TDNN + LSTM &  $\pm$  \\
		\bottomrule
	\end{tabular}
\end{table}

==> Sections/Table_Result_Multiclass.tex <==
\begin{table*}[ht!]
	\small
	\centering
	\caption{\textbf{Multi-Class Classification Result} of real-time seizure detection on TUH EEG dataset on CNN2D+LSTM, averaged over $5$ runs.}
	\label{Result}
	\begin{tabular}{c|ccccc}
		\toprule
		Methods & AUROC & AUPRC & F1 & TPR & TNR\\
		\midrule
		Generalized Seizure (GNSZ)  &  $\pm$  &  $\pm$  &  $\pm$  &  $\pm$  &  $\pm$  \\
		Focal Non-Specific seizure (FNSZ)  &  $\pm$  &  $\pm$  &  $\pm$  &  $\pm$  &  $\pm$  \\
		Simple Partial Seizure (SPSZ) &  $\pm$  &  $\pm$  &  $\pm$  &  $\pm$  &  $\pm$  \\
		Complex Partial Seizure (CPSZ) &  $\pm$  &  $\pm$  &  $\pm$  &  $\pm$  &  $\pm$  \\
		Absence Seizure (ABSZ) &  $\pm$  &  $\pm$  &  $\pm$  &  $\pm$  &  $\pm$  \\
		Tonic Seizure (TNSZ) &  $\pm$  &  $\pm$  &  $\pm$  &  $\pm$  &  $\pm$  \\
		Myoclonic Seizure (MYSZ) &  $\pm$  &  $\pm$  &  $\pm$  &  $\pm$  &  $\pm$  \\
		\midrule
		\textbf{Average} & \textbf{94.2 $\pm$ 0.3} &  \textbf{94.2 $\pm$ 0.3} &  \textbf{94.2 $\pm$ 0.3} &  \textbf{94.2 $\pm$ 0.3} &  \\ %exp setting with the best performance
		\bottomrule
	\end{tabular}
\end{table*}

==> Sections/Table_leads.tex <==
\begin{table*}[h!]
	\centering
 	\caption{Lead information for TUH datset}
	\label{leads}
	\begin{tabular}{c|c}
		\toprule
		Lead Type & Lead Info \\
		\midrule
		Unipolar Montage & FP1, FP2, F3, F4, F7, F8, C3, C4, CZ, T3, T4, P3, P4, O1, O2, T5, T6, PZ, FZ \\
		Bipolar Montage  & FP1-F7, F7-T3, T3-T5, T5-O1, FP2-F8, F8-T4, T4-T6, T6-O2, T3-C3, C3-CZ, CZ-C4 C4-T4, \\
		&FP1-F3, F3-C3, C3-P3, P3-O1, FP2-F4, F4-C4, C4-P4, P4-O2\\
		\bottomrule
	\end{tabular}
\end{table*}
